Theory of Stochastic Drift

In studying randomized search heuristics, a frequent quantity of interest is the first time a (real-valued) stochastic process obtains (or passes) a certain value. The processes under investigation commonly show a bias towards this goal, the \emph{stochastic drift}. Turning an iteration-wise expected bias into a first time of obtaining a value is the main result of \emph{drift theorems}. This thesis introduces the theory of stochastic drift, providing examples and reviewing the main drift theorems available. Furthermore, the thesis explains how these methods can be applied in various contexts, including those where drift theorems seem a counterintuitive choice. Later sections examine related methods and approaches.

==> LaTeXAuxiliaryDefinitions/core/general_commands.tex <==
% This file contains all sorts of macros that are globally used. Further, certain options made available through packages are set here as well.
%
% This file contains the following parts:
%   • Miscellaneous
%   • Footnotes
%   • Theorem Environments
%   • Meta Commands
%   • Common Commands


%%%%%%%%%%%%%%%%%%%
%% Miscellaneous %%
%%%%%%%%%%%%%%%%%%%

% Defines the layout of the title.
\date{}

% Defines the IfEmptyTF command. This is useful for optional arguments provided as [].
\makeatletter
    \def\IfEmptyTF#1%
    {%
        \if\relax\detokenize{#1}\relax%
            \expandafter\@firstoftwo%
        \else%
            \expandafter\@secondoftwo%
        \fi%
    }
\makeatother

% Creates an environment that automatically uses math mode if necessary and creates a space afterward if wanted. Basically, if the command \example is defined to use this environment, you can use \example without mathe mode in normal text as if it were ordinary text.
\NewDocumentCommand{\mathOrText}{m}
{%
    \ensuremath{#1}\xspace%
}

% Reduces the space around scaling bracekts.
\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}

% Lets math text in an environment of bold text also appear bold.
\makeatletter
    \DeclareRobustCommand{\bfseries}%
    {%
        \not@math@alphabet\bfseries\mathbf%
        \fontseries\bfdefault\selectfont%
        \boldmath%
    }


% Adds square and curly brackets to the exceptions for xspace such that no space is used right in front of them.
\xspaceaddexceptions{]\}}

% Formats URLs by using the normal font (not the typewriter font).
\urlstyle{rm}

% Allows large display formulas to span multiple pages.
\allowdisplaybreaks

% Defines an optional argument for labels named ›ineq‹ that signals that cleveref should name the respective reference ›inequality‹ instead of its actual name.
\crefname{ineq}{inequality}{inequalities}
\creflabelformat{ineq}{#2{\upshape(#1)}#3}

% Defines an optional argument for labels named ›term‹ that signals that cleveref should name the respective reference ›term‹ instead of its actual name.
\crefname{term}{term}{terms}
\creflabelformat{term}{#2{\upshape(#1)}#3}

% Defines an optional argument for labels named ›cond‹ that signals that cleveref should name the respective reference ›condition‹ instead of its actual name.
\crefname{cond}{condition}{conditions}
\creflabelformat{term}{#2{\upshape(#1)}#3}


%%%%%%%%%%%%%%%
%% Footnotes %%
%%%%%%%%%%%%%%%

% Remove the footnote rule.
\setfootnoterule{0 cm}

% The footnote number is made bold and not in superscript.
\deffootnote[1.2 em]{1.2 em}{0 em}{\makebox[1.4 em][l]{\textbf{\thefootnotemark}}}

% In the following, the command ›footnote‹ is redefined such that the footnote mark can be more easily adjusted.
\let\oldfootnote\footnote

% The following are variables used by the command.
\newlength{\spaceBeforeFootnote} % Denotes the space before the footnote mark in em.
\newlength{\spaceAfterFootnote}  % Denotes the space after the footnote mark in em.

% The new footnote command. The first three arguments are optional, the fourth mandatory. Its arguments have the following meaning:
%   1. The amount of space before the footnote mark in em. The default is 0.
%   2. The amount of space after the footnote mark in em. The default is 0.
%   3. The number of the footnote mark.
%   4. The text of the footnote.
\RenewDocumentCommand{\footnote}{o o o m}%
{%
    \IfNoValueTF{#1}%
    {%
        \oldfootnote{#4}%
    }%
    {%
        \setlength{\spaceBeforeFootnote}{\IfEmptyTF{#1}{0}{#1} em}%
        \IfNoValueTF{#2}%
        {%
            \hspace*{\spaceBeforeFootnote}\oldfootnote{#4}%
        }%
        {%
            \setlength{\spaceAfterFootnote}{\IfEmptyTF{#2}{0}{#2} em}%
            \hspace*{\spaceBeforeFootnote}\IfNoValueTF{#3}{\oldfootnote{#4}}{\oldfootnote[#3]{#4}}\hspace*{\spaceAfterFootnote}%
        }%
    }%
}

% The following commands enable it such that footnotes can be used in various other environments other than simple text.
\makesavenoteenv{figure}
\makesavenoteenv{table}
\makesavenoteenv{tabular}


%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Theorem Environments %%
%%%%%%%%%%%%%%%%%%%%%%%%%%

% The following theorem style uses a bold heading for the theorem and normal (upright) text. The environment begins with a triangle of color ›stroke1‹ pointing to the right and uses a QED symbol that is a triangle of the same color pointing to the left. Thus, the environment is enclosed by triangles.
\declaretheoremstyle
[
   	spaceabove = \topsep,
   	spacebelow = \topsep,
   	headfont = \bfseries,
   	headformat = \textcolor{stroke1}{$\blacktriangleright$} \NAME~\NUMBER \NOTE,
   	notefont = \bfseries,
   	notebraces = {(}{)},
   	bodyfont = \normalfont,
   	postheadspace = 0.5 em,
   	qed = \textcolor{stroke1}{\bfseries$\blacktriangleleft$},
]
{myTheoremStyle}


\declaretheoremstyle[
   	spaceabove = 2pt,
   	spacebelow = \topsep,
   	headfont = \bfseries,
   	headformat = \textcolor{stroke1}{$\blacktriangleright$} \NAME~\NUMBER \NOTE,
   	notefont = \bfseries,
   	notebraces = {(}{)},
   	bodyfont = \normalfont,
   	postheadspace = 0.5 em,
   	qed = \textcolor{stroke1}{\bfseries$\blacktriangleleft$},
	mdframed={
	  skipabove=8pt,
	  skipbelow=6pt,
	  hidealllines=true,
	  backgroundcolor={gray!15},
	  innerleftmargin=10pt,
	  innerrightmargin=10pt}
]{myTheoremStyleShaded}

% The QED symbol used in proofs is a squre with color ›stroke1‹ in order to look similar to the theorem environments.
\renewcommand*{\qedsymbol}{\textcolor{stroke1}{$\blacksquare$}}

\declaretheorem
[
    style = myTheoremStyle,
    name = Conjecture,
    numberwithin = section,
]
{conjecture}
\declaretheorem
[
    style = myTheoremStyle,
    name = Proposition,
    sharenumber = conjecture,
]
{proposition}
\declaretheorem
[
   	style = myTheoremStyle,
   	name = Claim,
     sharenumber = conjecture,
]
{claim}
% \declaretheorem
% [
%    	style = myTheoremStyle,
%    	name = Lemma,
%     sharenumber = conjecture,
% ]
% {lemma}
\declaretheorem
[
   	style = myTheoremStyle,
   	name = Corollary,
     sharenumber = conjecture,
]
{corollary}
\declaretheorem
[
   	style = myTheoremStyle,
   	name = Theorem,
     sharenumber = conjecture,
]
{theorem}
\declaretheorem
[
   	style = myTheoremStyleShaded,
   	name = Definition,
     sharenumber = conjecture,
]
{definition}
\declaretheorem
[
    style = myTheoremStyle,
    name = Example,
    sharenumber = conjecture,
]
{example}
% \declaretheorem
% [
%     style = myTheoremStyle,
%     name = Remark,
%     sharenumber = conjecture,
% ]
% {remark}
% \declaretheorem
% [
%     style = myTheoremStyle,
%     name = Exercise,
% ]
% {exercise}
\declaretheorem[
    style = myTheoremStyleShaded,
    name = Satz,
    sharenumber = conjecture,
]
{satz}
\declaretheorem[
    style = myTheoremStyle,
    name = Lemma,
    sharenumber = conjecture,
]
{lemma}
\declaretheorem[
    style = myTheoremStyle,
    name = Beispiel,
    sharenumber = conjecture,
]
{beispiel}
\declaretheorem[
    style = myTheoremStyle,
    name = Aufgabe
]
{exercise}
\declaretheorem[
    style = myTheoremStyle,
    name = Vorbereitung
]
{prep}
\declaretheorem[
    style = myTheoremStyle,
    name = Lösung
]
{solution}
\declaretheorem[
    style = myTheoremStyle,
    name = Bepunktung
]
{points}
\declaretheorem[
    style = myTheoremStyle,
    name = Bonusaufgabe
]
{bonus}
\declaretheorem
[
    style = myTheoremStyle,
    name = Kommentar,
    sharenumber = conjecture,
]
{remark}
\declaretheorem[
    style = myTheoremStyle,
    name = Bemerkung,
    sharenumber = conjecture,
]
{note}

\newcommand{\inlineComment}[1]{\textcolor{darkblue}{[Kommentar: #1]}}

%%%%%%%%%%%%%%%%%%%
%% Meta Commands %%
%%%%%%%%%%%%%%%%%%%

% A template for a function that can use an optional variable bracket size. Its arguments have the following meaning:
%   1. The name of the function.
%   2. The type of the left bracket. This should be a bracket symbol, as it will be forwarded to the command \left.
%   3. The type of the right bracket. The same restrictions as with parameter 2 hold here.
%   4. The arguments that the function takes, that is, the things that are enclosed by the brackets.
%   5. The size of the brackets. This should be a value like \big or similar, as it will be forwarded to the command \left.
\NewDocumentCommand{\functionTemplate}{m m m m o}%
{%
    \IfNoValueTF{#5}%
    {%
        \mathOrText{#1\left#2{#4}\right#3}%
    }%
    {%
        \mathOrText{#1#5#2{#4}#5#3}%
    }%
}

% The following two commands are used as variables for the following command.
\newcommand*{\leftBracketType}{(}
\newcommand*{\rightBracketType}{)}

% This is a command that creates a command that is a function as defined by the command \functionTemplate. Its arguments have the following meaning:
%   1. The name of the function command.
%   2. The name of the function itself.
%   3. The type of the left bracket. This will be forwarded to parameter 2 of \functionTemplate. The default is (. Use \lbrack for [ and \{ for }.
%   4. The type of the right bracket. This will be forwarded to parameter 3 of \functionTemplate. The default is ). The rest is similar to parameter 3.
% The command created has two optional arguments, which are as follows:
%   1. The arguments of the function. If this is empty, only the name of the function will be used.
%   2. The size of the brackets. This will be forwarded to parameter 5 of \functionTemplate.
\NewDocumentCommand{\createFunction}{m m o o}%
{%
    \renewcommand*{\leftBracketType}{\IfNoValueTF{#3}{(}{#3}}%
    \renewcommand*{\rightBracketType}{\IfNoValueTF{#4}{)}{#4}}%
    \NewDocumentCommand{#1}{o o}%
    {%
        \IfNoValueTF{##1}%
        {%
            \mathOrText{#2}%
        }%
        {%
            \functionTemplate{#2}{\leftBracketType}{\rightBracketType}{##1}[##2]%
        }%
    }%
}

% A template for a probabilistic symbol, which can make use of a condition denoted by |. Its arguments have the following meaning:
%   1. The name of the function.
%   2. The argument of the function.
%   3. The condition of the function. The default is that there is no condition.
%   4. The size of the brackets. This will be forwarded to parameter 5 of \functionTemplate.
\DeclareDocumentCommand{\probabilisticFunctionTemplate}{m m O{} o}
{%
    \functionTemplate{#1}%
    {\lbrack}%
    {\rbrack}%
    {#2\IfEmptyTF{#3}{}{\ \IfNoValueTF{#4}{\left}{#4}\vert\ \vphantom{#2}#3\IfNoValueTF{#4}{\right.}{}}}%
    [#4]%
}


%%%%%%%%%%%%%%%%%%%%%
%% Common Commands %%
%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%
% Number Sets

% Number sets appear in bold by default.
\newcommand*{\N}{\mathOrText{\mathbf{N}}}
\newcommand*{\Z}{\mathOrText{\mathbf{Z}}}
\newcommand*{\Q}{\mathOrText{\mathbf{Q}}}
\newcommand*{\R}{\mathOrText{\mathbf{R}}}
\newcommand*{\C}{\mathOrText{\mathbf{C}}}
\newcommand*{\indicatorFunctionSymbol}{\mathbf{1}}

%%%%%%%%%%%%%%%%%%%%%
% Probabilistic Functions
% All of these functions follow the outline of \probabilisticFunctionTemplate. That is, the syntax is, for example, \Pr{A}[B][\big], which would be shown as Pr[A | B] with \big brackets.

% Probability measure
\RenewDocumentCommand{\Pr}{m O{} o}%
{%
    \probabilisticFunctionTemplate{\mathrm{Pr}}{#1}[#2][#3]%
}

% Expected value
\NewDocumentCommand{\E}{m O{} o}%
{%
    \probabilisticFunctionTemplate{\mathrm{E}}{#1}[#2][#3]%
}

% Variance
\NewDocumentCommand{\Var}{m O{} o}%
{%
    \probabilisticFunctionTemplate{\mathrm{Var}}{#1}[#2][#3]%
}

%%%%%%%%%%%%%%%%%%%%%
% Landau Notation
% The following commands all take a mandatory argument, which is the term of the Landau notation, as well as an optional argument, which determines the size of the brackets.

% Big O
\DeclareDocumentCommand{\bigO}{m o}%
{%
    \functionTemplate{\mathrm{O}}{(}{)}{#1}[#2]%
}

% Small O
\DeclareDocumentCommand{\smallO}{m o}%
{%
    \functionTemplate{\mathrm{o}}{(}{)}{#1}[#2]%
}

% Big Theta
\DeclareDocumentCommand{\bigTheta}{m o}%
{%
    \functionTemplate{\upTheta}{(}{)}{#1}[#2]%
}

% Big Omega
\DeclareDocumentCommand{\bigOmega}{m o}%
{%
    \functionTemplate{\upOmega}{(}{)}{#1}[#2]%
}

% Small Omega
\DeclareDocumentCommand{\smallOmega}{m o}%
{%
    \functionTemplate{\upomega}{(}{)}{#1}[#2]%
}

%%%%%%%%%%%%%%%%%%%%%
% Constants

% Pi; ratio of a circle’s circumference to its diameter
\newcommand*{\circlePi}{\mathOrText{\uppi}}

% Euler’s constant. This command takes an optional parameter, which becomes the exponent of this constant.
\DeclareDocumentCommand{\eulerE}{o}%
{%
    \mathOrText{\mathrm{e}\IfNoValueTF{#1}{}{^{#1}}}%
}

% i; the imaginary unit
\newcommand*{\imaginaryUnit}{\mathOrText{\mathrm{i}}}

%%%%%%%%%%%%%%%%%%%%%
% Other

% A polynomial function. The mandatory parameter is the argument of the function, the optional one is the size of the brackets.
\DeclareDocumentCommand{\poly}{m o}%
{%
    \functionTemplate{\mathrm{poly}}{(}{)}{#1}[#2]%
}

% The identity function
\createFunction{\id}{\mathrm{id}}

% An indicator function. The first parameter is set as an index, the second is the argument of the function, and the third is the size of the brackets.
\NewDocumentCommand{\ind}{m o o}%
{%
    \IfNoValueTF{#2}%
    {%
        \mathOrText{\indicatorFunctionSymbol_{#1}}%
    }%
    {%
        \functionTemplate{\indicatorFunctionSymbol_{#1}}{(}{)}{#2}[#3]%
    }%
}

% The domain of a function. Its parameters are the same as for \poly.
\DeclareDocumentCommand{\dom}{m o}%
{%
    \functionTemplate{\mathrm{dom}}{(}{)}{#1}[#2]%
}

% The range of a function. Its parameters are the same as for \poly.
\DeclareDocumentCommand{\rng}{m o}%
{%
    \functionTemplate{\mathrm{rng}}{(}{)}{#1}[#2]%
}

% The d for an integral. The optional parameter becomes the exponent/degree of the operator.
\DeclareDocumentCommand{\d}{o}%
{%
    \mathrm{d}\IfNoValueTF{#1}{}{^{#1}}%
}

% A command that creates sets. The first parameter is the left-hand side, the second is the right-hand side, and the third (optional) parameter is the size of the brackets.
\DeclareDocumentCommand{\set}{m m o}%
{%
    \mathOrText{\IfNoValueTF{#3}{\left}{#3}\{#1\ \IfNoValueTF{#3}{\left}{#3}\vert\ \vphantom{#1}#2\IfNoValueTF{#3}{\right.}{}\IfNoValueTF{#3}{\right}{#3}\}}%
}

\input{Template/packages_and_commands/additional_commands.tex}

==> LaTeXAuxiliaryDefinitions/core/standard_packages.tex <==
% This file contains most of the packages used for this document. If you want to add a package, do it here.
% Some packages are already included in other files in the ›core‹ folder if they were already necessary. Thus, make sure to go through these files too if you want to know whether a certain package is already included.
%
% This file contains the following parts:
%   • Typography
%   • Colors
%   • Math
%   • Fonts
%   • Graphics
%   • Tables
%   • Enumerations
%   • Algorithms
%   • Spaces and Special Characters
%   • Miscellaneous
%   • Bibliography
%   • Additional Packages
%   • Hyperlinks

%%%%%%%%%%%%%%%%
%% Typography %%
%%%%%%%%%%%%%%%%

\usepackage[ngerman]{babel} %american
\usepackage
[
    babel = true, % Enables language-specific tuning.
]
{microtype}           % Uses the text space more efficiently.
\usepackage{csquotes} % Uses the correct quotes according to the current language.


%%%%%%%%%%%%
%% Colors %%
%%%%%%%%%%%%

\usepackage
[
    dvipsnames,
    table,
]{xcolor} % Allows it to define colors. The option says that common names can be used.

% Dark blue.
\definecolor{stroke1}{HTML}{2574A9} % This color is used as the standard color to highlight things.


%%%%%%%%%%
%% Math %%
%%%%%%%%%%

% The following packages are the standard packages used in order to typeset math. They contain a lot of useful commands.
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{thmtools}
\usepackage{mathtools}
\usepackage{thm-restate}
\usepackage{dsfont}        % Yields far better blackboard-bold letters than \mathbb. Use \mathds in order to write such letters.
\usepackage{Template/braceMnSymbol} % Adjusts overbraces and underbraces such that longer versions are put together seamlessly.


%%%%%%%%%%%
%% Fonts %%
%%%%%%%%%%%

\usepackage
[
    ttscale = 0.85, % Scales the typewriter font.
]
{libertine} % The main font used in this thesis.
\usepackage
[
    libertine,    % Changes the math font to libertine (the main font).
    slantedGreek, % Makes all greek letters italic by default. If you want to use an upright greek letter, use ›\up‹ immediately followed by the letter’s name. For example, \upGamma displays an upright uppercase gamma.
    vvarbb,       % Changes the \mathbb font to another font. However, \mathbb remains ugly and should not be used. Use \mathds instead.
    libaltvw,     % Uses different characters for v und w that look far better than the default ones.
]
{newtxmath} % The main math font of this thesis. It fits well with the main font.
\usepackage{url} % Responsible for URL formatting.
\usepackage{bm}  % Allows to use sensible bold letters in math mode. This package has to go after the font packages. Otherwise it does not work correctly!


%%%%%%%%%%%%%%
%% Graphics %%
%%%%%%%%%%%%%%

\usepackage{graphicx} % The standard package for including graphics into your document.
\usepackage
[
    subrefformat = simple, % Formats the label of the \subref command without parentheses.
    labelformat = simple,  % Formats the mark of a subfigure without parentheses.
]
{subcaption}         % Enables it to have subfigures inside of a single figure.


%%%%%%%%%%%%
%% Tables %%
%%%%%%%%%%%%

\usepackage{array}     % Improves the way that tables can be formatted.
\usepackage{booktabs}  % Adds lines (called ›rules‹) that can be used in tables and improves spacing.
\usepackage{longtable} % Allows to make tables that span multiple pages.
\usepackage{pdflscape} % Allows to change a page into landscape. This is handy if a table is very wide.


%%%%%%%%%%%%%%%%%%
%% Enumerations %%
%%%%%%%%%%%%%%%%%%

\usepackage{enumitem} % Adds tons of useful features to enumeration environments.


%%%%%%%%%%%%%%%%
%% Algorithms %%
%%%%%%%%%%%%%%%%

\usepackage
[
    ngerman,
    ruled,         % Creates lines at the top and at the bottom. Further, the caption is now above the algorithm.
    vlined,        % Shows the scope of a statement spanning multiple lines via a small vertical bar. Thus, no closing tags are needed.
    linesnumbered, % Shows line numbers.
    algo2e
]
{algorithm2e} % Allows to write pseudocode.
\DontPrintSemicolon
\SetAlgoCaptionLayout{leftline}
\LinesNumbered
\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Spaces and Special Characters %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{xspace}   % Adds the functionality that a space after a command will be shown as a space in the output.
\usepackage
[
    shortcuts, % Allows to use short symbols for non-breaking hyphens and dashes instead of lengthy commands.
]
{extdash}             % Adds non-breaking hyphens and dashes.
\usepackage{setspace} % Allows to easily chnage the spacing inside of the document.


%%%%%%%%%%%%%%%%%%%
%% Miscellaneous %%
%%%%%%%%%%%%%%%%%%%

\usepackage{xparse}    % Is used in order to define reasonable commands.
\usepackage{footnote}  % Allows it to extend the environments footnotes can be used in. It is said that this package is in conflict with ›hyperref‹. I did not note any troubles. However, if something is fishy, it is probably best to not use this package.
\usepackage{afterpage} % Adds the \afterpage command, which specifies that the provided argument shall be processed after the current page is finished.
\usepackage
[
    textsize = scriptsize, % Determines the text size of the TODO note.
]
{todonotes}            % Adds TODO notes to the document. These are small text areas inside of the margin of a page.


%%%%%%%%%%%%%%%%%%
%% Bibliography %%
%%%%%%%%%%%%%%%%%%

\usepackage
[
    sortcites,              % Sort multiple references when citing them together.
    style = alphabetic,     % The style of a citation mark.
    defernumbers,           % Makes sure that references always have unique numbers. This is important if you use multiple bibliographies.
    safeinputenc,           % Allows to use UTF8 characters in the bibliography and tries to translate them into TeX automatically.
    backref = true,         % Creates back references in the bibliography.
    backrefstyle = three,   % Compresses three or more consecutive pages in the back references into a range.
    hyperref = true,        % Makes links generated by biblatex clickable. If hyperref is not used, a warning is issued.
    maxbibnames = 99,       % The maximum number of names displayed in the bibliography.
    maxcitenames = 2,       % The maximum number of names displayed when using commands like ›textcite‹. The default is 3. After that, ›et al.‹ is used.
%    useprefix,              % Prints name prefixes, such as ›von‹. The default is false. This means that prefixes are not considered to be part of the last name.
]
{biblatex} % Used in order to format the bibliography.

\DefineBibliographyStrings{english}%
{%
    backrefpage  = {\lowercase{s}ee page}, % For a single page number.
    backrefpages = {\lowercase{s}ee pages} % For multiple page numbers.
}

\DeclareFieldFormat{titlecase}{\MakeSentenceCase*{#1}}

\addbibresource{references.bib}


%%%%%%%%%%%%%%%%%%%%%%%%%
%% Additional Packages %%
%%%%%%%%%%%%%%%%%%%%%%%%%

\input{Template/packages_and_commands/additional_packages}


%%%%%%%%%%%%%%%%
%% Hyperlinks %%
%%%%%%%%%%%%%%%%
\definecolor{darkblue}{rgb}{0, 0, 0.5}

\usepackage
[
    bookmarks = true,                 % Generates boodmarks for the PDF.
    bookmarksopen = false,            % The bookmarks are closed by default.
    bookmarksnumbered = true,         % The bookmarks use the numbers of the corresponding headline.
    pdfstartpage = 1,                 % The first page seen when opening the PDF.
    colorlinks = true,                % The text of hyperlinks is colored instead of having a colored box around it.
    allcolors = stroke1,              % Every hyperlink uses the same color. If you want to change specific colors, use the commands below.
%        linkcolor = stroke1,          % The color of an in-document hyperlink.
%        citecolor = stroke1,          % The color of a citation.
%        filecolor = stroke1,          % The color of a file link.
%        pagecolor = stroke1,          % The color of a reference to a page.
%        urlcolor = stroke1,           % The color of a weblink.
    breaklinks = true,
    linkcolor = darkblue,
    anchorcolor = darkblue,
    citecolor = darkblue,
    filecolor = darkblue,
    menucolor = darkblue,
    pagecolor = darkblue,
    urlcolor = darkblue
]
{hyperref} % The standard package that is used for creating hyperlinks inside of a document.

\usepackage
[
%    capitalise, % Capitalizes the words in front of the labels. This can also be done by simply using \Cref instead of \cref. In order to have a greater variety, this option is not used.
    noabbrev,   % The words in front of the labels are not abbreviated.
    nameinlink, % Extends the link of a reference to the word in front of it.
]
{cleveref} % This package must be included after ›hyperref‹. It creates clever references that know what they refer to.


==> LaTeXAuxiliaryDefinitions/header/header.tex <==
\vspace*{-10 ex}\noindent\printAuthor\vspace*{-3 ex}

\hfill\includegraphics[height = 1.9 cm]{Template/header/logo_up.pdf}
\hspace*{1 em} \includegraphics[height = 1.9 cm]{Template/header/logo_hpi.pdf}
\vspace*{-4 ex}

{\noindent\Huge \printTitle}\\
\rule{\textwidth}{1 pt}\vspace*{1 ex}

\noindent
\begin{minipage}[t]{0.5\textwidth}
    \printLecture
\end{minipage}
\begin{minipage}[t]{0.5\textwidth}
    \begin{raggedleft}
    		\printHandInDate

        \printHandInDateQuiz

        \printHandInDatePrep

        \printHandInDateRiddle

        \printHandInDateBonus

        \printHandInNote
        
    \end{raggedleft}
\end{minipage}\\[1.5 ex]
\rule{\textwidth}{1 pt}


\bigskip

==> LaTeXAuxiliaryDefinitions/header/header_format.tex <==
\lohead[\normalfont\printLectureShort]{}
\rohead[\normalfont\printTerm]{}
\cohead{}
\cofoot*{}
\cofoot*{\normalfont\thepage{}~/~\pageref{LastPage}}

\pagestyle{plain.scrheadings}

==> LaTeXAuxiliaryDefinitions/headerOld.tex <==
% This file contains all sorts of macros that are globally used. Further, certain options made available through packages are set here as well.
%
% This file contains the following parts:
%   • Miscellaneous
%   • Footnotes
%   • Theorem Environments
%   • Meta Commands
%   • Common Commands


%%%%%%%%%%%%%%%%%%%%%%%%
% Macros for the title %
%%%%%%%%%%%%%%%%%%%%%%%%

% The name of the authors.
\newcommand*{\printAuthor}{}
\newcommand*{\authorName}[1]{\renewcommand*{\printAuthor}{#1}}

% The name of the document.
\newcommand*{\printTitle}{}
\newcommand*{\titleName}[1]{\renewcommand*{\printTitle}{#1}}


% Potentially a subtitle.
\newcommand*{\printSubTitle}{}
\newcommand*{\subTitleName}[1]{\renewcommand*{\printSubTitle}{{\Large #1} \\}}

% Auxiliary Information.
\newcommand*{\printInformation}{}
\newcommand*{\infoName}[1]{\renewcommand*{\printInformation}{#1}}


% The version.
\newcommand*{\printVersion}{}
\newcommand*{\versionName}[1]{\renewcommand*{\printVersion}{#1}}


% The maker version.
\newcommand*{\printmakerVersion}{}
\newcommand*{\makerVersionName}[1]{\renewcommand*{\printmakerVersion}{#1}}


%%%%%%%%%%%%%%%%%%%
%% Miscellaneous %%
%%%%%%%%%%%%%%%%%%%

% Defines the layout of the title.
\date{}

% Defines the IfEmptyTF command. This is useful for optional arguments provided as [].
\makeatletter
    \def\IfEmptyTF#1%
    {%
        \if\relax\detokenize{#1}\relax%
            \expandafter\@firstoftwo%
        \else%
            \expandafter\@secondoftwo%
        \fi%
    }
\makeatother

% Creates an environment that automatically uses math mode if necessary and creates a space afterward if wanted. Basically, if the command \example is defined to use this environment, you can use \example without mathe mode in normal text as if it were ordinary text.
\NewDocumentCommand{\mathOrText}{m}
{%
    \ensuremath{#1}\xspace%
}

% Reduces the space around scaling bracekts.
\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}

% Lets math text in an environment of bold text also appear bold.
\makeatletter
    \DeclareRobustCommand{\bfseries}%
    {%
        \not@math@alphabet\bfseries\mathbf%
        \fontseries\bfdefault\selectfont%
        \boldmath%
    }


% Adds square and curly brackets to the exceptions for xspace such that no space is used right in front of them.
\xspaceaddexceptions{]\}}

% Formats URLs by using the normal font (not the typewriter font).
\urlstyle{rm}

% Allows large display formulas to span multiple pages.
\allowdisplaybreaks

% Defines an optional argument for labels named ›ineq‹ that signals that cleveref should name the respective reference ›inequality‹ instead of its actual name.
\crefname{ineq}{inequality}{inequalities}
\creflabelformat{ineq}{#2{\upshape(#1)}#3}

% Defines an optional argument for labels named ›term‹ that signals that cleveref should name the respective reference ›term‹ instead of its actual name.
\crefname{term}{term}{terms}
\creflabelformat{term}{#2{\upshape(#1)}#3}

% Defines an optional argument for labels named ›cond‹ that signals that cleveref should name the respective reference ›condition‹ instead of its actual name.
\crefname{cond}{condition}{conditions}
\creflabelformat{term}{#2{\upshape(#1)}#3}


%%%%%%%%%%%%%%%
%% Footnotes %%
%%%%%%%%%%%%%%%

% Remove the footnote rule.
\setfootnoterule{0 cm}

% The footnote number is made bold and not in superscript.
\deffootnote[1.2 em]{1.2 em}{0 em}{\makebox[1.4 em][l]{\textbf{\thefootnotemark}}}

% In the following, the command ›footnote‹ is redefined such that the footnote mark can be more easily adjusted.
\let\oldfootnote\footnote

% The following are variables used by the command.
\newlength{\spaceBeforeFootnote} % Denotes the space before the footnote mark in em.
\newlength{\spaceAfterFootnote}  % Denotes the space after the footnote mark in em.

% The new footnote command. The first three arguments are optional, the fourth mandatory. Its arguments have the following meaning:
%   1. The amount of space before the footnote mark in em. The default is 0.
%   2. The amount of space after the footnote mark in em. The default is 0.
%   3. The number of the footnote mark.
%   4. The text of the footnote.
\RenewDocumentCommand{\footnote}{o o o m}%
{%
    \IfNoValueTF{#1}%
    {%
        \oldfootnote{#4}%
    }%
    {%
        \setlength{\spaceBeforeFootnote}{\IfEmptyTF{#1}{0}{#1} em}%
        \IfNoValueTF{#2}%
        {%
            \hspace*{\spaceBeforeFootnote}\oldfootnote{#4}%
        }%
        {%
            \setlength{\spaceAfterFootnote}{\IfEmptyTF{#2}{0}{#2} em}%
            \hspace*{\spaceBeforeFootnote}\IfNoValueTF{#3}{\oldfootnote{#4}}{\oldfootnote[#3]{#4}}\hspace*{\spaceAfterFootnote}%
        }%
    }%
}

% The following commands enable it such that footnotes can be used in various other environments other than simple text.
\makesavenoteenv{figure}
\makesavenoteenv{table}
\makesavenoteenv{tabular}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% HEADER


\lohead[\normalfont\printTitle]{}
\rohead[\normalfont\printInformation]{}
\cohead{}
\cofoot*{}
\cofoot*{\normalfont\thepage{}~/~\pageref{LastPage}}

\pagestyle{plain.scrheadings}

\newcommand{\makeHeader}{
\thispagestyle{scrheadings}

\vspace*{-10 ex}\noindent\printAuthor\vspace*{-3 ex}

\hfill\includegraphics[height = 1.9 cm]{../../templates/LaTeXAuxiliaryDefinitions/header/logo_up.pdf}
\hspace*{1 em} \includegraphics[height = 1.9 cm]{../../templates/LaTeXAuxiliaryDefinitions/header/logo_hpi.pdf}
\vspace*{-4 ex}

{\noindent\Huge \printTitle}\\
\printSubTitle
\rule{\textwidth}{1 pt}\vspace*{1 ex}

\noindent%
Compiled on \today\ 

\noindent%
\rule{\textwidth}{1 pt}


\bigskip}

==> LaTeXAuxiliaryDefinitions/packages_and_commands/additional_commands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%
% Macros for the title %
%%%%%%%%%%%%%%%%%%%%%%%%

% The name of the authors.
\newcommand*{\printAuthor}{}
\newcommand*{\authorName}[1]{\renewcommand*{\printAuthor}{#1}}

% The name of the document.
\newcommand*{\printTitle}{}
\newcommand*{\titleName}[1]{\renewcommand*{\printTitle}{#1}}

% The name of the lecture.
\newcommand*{\printLecture}{}
\newcommand*{\lectureName}[1]{\renewcommand*{\printLecture}{#1}}

% The name of the lecture in short format.
\newcommand*{\printLectureShort}{}
\newcommand*{\lectureNameShort}[1]{\renewcommand*{\printLectureShort}{#1}}

% The name of the term.
\newcommand*{\printTerm}{}
\newcommand*{\termName}[1]{\renewcommand*{\printTerm}{#1}}

% The name of the term.
\newcommand*{\printHandInDate}{}
\newcommand*{\dateToHandIn}[1]{\renewcommand*{\printHandInDate}{Alle Aufgaben bis \textbf{#1}}}

\newcommand*{\printHandInDateQuiz}{}
\newcommand*{\dateToHandInQuiz}[1]{\renewcommand*{\printHandInDateQuiz}{Verständnisquiz (Moodle) bis \textbf{#1}}}

\newcommand*{\printHandInDatePrep}{}
\newcommand*{\dateToHandInPrep}[1]{\renewcommand*{\printHandInDatePrep}{Vorbereitungsaufgaben bis \textbf{#1}}}

\newcommand*{\printHandInDateRiddle}{}
\newcommand*{\dateToHandInRiddle}[1]{\renewcommand*{\printHandInDateRiddle}{Beweis-/ Knobelaufgaben bis \textbf{#1}}}

\newcommand*{\printHandInDateBonus}{}
\newcommand*{\dateToHandInBonus}[1]{\renewcommand*{\printHandInDateBonus}{Bonusaufgaben bis \textbf{#1}}}

% The name of the term.
\newcommand*{\printHandInNote}{}
\newcommand*{\handInLocation}[1]{\renewcommand*{\printHandInNote}{#1}}


%%%%%%%%%%
% Format %
%%%%%%%%%%

\newcommand*{\infobox}[1]
{%
    \begin{tabular}{!{\color{stroke1}\vrule width 2pt}p{\textwidth - 1.5 em}!{\color{gray!15}\vrule width 2pt}}%
        \rowcolor{gray!15}\vspace*{-5 pt}%
        #1%
        \vspace*{2.5 pt}%
    \end{tabular}%
    \bigskip%
}


%%%%%%%%%%%%%%%
% Other stuff %
%%%%%%%%%%%%%%%

% Indicator function
\newcommand*{\indicator}[1]{\mathOrText{\mathbf{1}{\{#1\}}}}

% Random process
\DeclareDocumentCommand{\randomProcess}{m o}
{%
    \mathOrText{X^{(#1)}\IfNoValueTF{#2}{}{_{#2}}}%
}

% Transformed process
\DeclareDocumentCommand{\transformedProcess}{o}
{%
    \mathOrText{Y\IfNoValueTF{#1}{}{_{#1}}}%
}

% Filtration
\DeclareDocumentCommand{\filtration}{o}
{%
    \mathOrText{\mathcal{F}\IfNoValueTF{#1}{}{_{#1}}}%
}

%\newcommand*{\N}{\mathOrText{\mathbf{N}}}
%\newcommand*{\R}{\mathOrText{\mathbf{R}}}
\newcommand*{\timePoint}{\mathOrText{t}}
\newcommand*{\stoppingTime}{\mathOrText{T}}
\newcommand*{\target}{\mathOrText{\alpha}}
\newcommand*{\drift}{\mathOrText{\delta}}
\newcommand*{\driftPositive}{\mathOrText{\delta^+}}
\newcommand*{\driftNegative}{\mathOrText{\delta^-}}
\newcommand*{\defeq}{\mathOrText{\coloneqq}}
\newcommand*{\eqdef}{\mathOrText{\eqqcolon}}
\newcommand*{\numberOfProcesses}{\mathOrText{k}}


% Vanja:
\renewcommand\thebonus{B\arabic{bonus}}
%\counterwithin*{equation}{exercise}

\renewcommand{\labelenumi}{(\alph{enumi})}
\renewcommand{\labelenumii}{(\roman{enumii})}

\newcommand*{\Oh}{\mathrm{O}}
\newcommand*{\Na}{\mathbb{N}}
\newcommand*{\Ra}{\mathbb{Q}}
\renewcommand*{\Re}{\mathbb{R}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand*{\goed}{\textrm{göd}}
\newcommand*{\img}{\mathrm{img}}
\newcommand*{\myBigO}{\mathcal{O}}
% \newcommand*{\bigOmega}{\Omega}
% \newcommand*{\smallO}{\mathrm{o}}
% \newcommand*{\smallOmega}{\upomega}


\newcommand{\makeCompact}{%
\setlength{\itemsep}{1pt}%
\setlength{\parsep}{0pt}%
\setlength{\parskip}{0pt}}

\newcommand{\comment}[1]{\textcolor{blue}{[#1]}}
\newcommand{\ignore}[1]{}

% \newcommand{\set}[2]{\{ #1 \mid #2 \}}
\newcommand{\natnum}{\mathbb{N}}
\newcommand{\rationals}{\mathbb{Q}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\realnum}{\mathbb{R}}
\newcommand{\Bij}{\mathcal{B}}

\newcommand{\isom}{\cong}

\newcommand{\FrakA}{\mathfrak{A}}
\newcommand{\converges}{\mathclose{\hbox{$\downarrow$}}}
\newcommand{\diverges}{\mathclose{\hbox{$\uparrow$}}}
\newcommand{\CalA}{\mathcal{A}}
\newcommand{\CalC}{\mathcal{C}}
\newcommand{\CalF}{\mathcal{F}}
\newcommand{\CalG}{\mathcal{G}}
\newcommand{\CalP}{\mathcal{P}}
\newcommand{\CalM}{\mathcal{M}}
\newcommand{\CalN}{\mathcal{N}}
\newcommand{\CalR}{\mathcal{R}}
\newcommand{\CalS}{\mathcal{S}}
\newcommand{\CalX}{\mathcal{X}}

% \newcommand{\id}{\mathrm{id}}
\newcommand{\pad}{\mathrm{pad}}
% \newcommand{\dom}{\mathrm{dom}}
%\newcommand{\modulo}{\; \mathrm{mod}}
\newcommand{\range}{\mathrm{range}}
\newcommand{\pair}[1]{\langle #1 \rangle}

\newcommand{\unpair}{\mathrm{unpair}}

\newcommand{\eqnComment}[2]{\underset{{\scriptstyle \text{#1}}}{#2}}

\DeclareMathOperator{\modulo}{mod}
\DeclareMathOperator{\Pow}{Pow}

==> LaTeXAuxiliaryDefinitions/packages_and_commands/additional_packages.tex <==
\usepackage{scrlayer-scrpage}
\usepackage{lastpage}

\usepackage{mdframed}
%\usepackage[theorems]{tcolorbox}

\usepackage[normalem]{ulem}

\usepackage{listings}
\lstset{%
    mathescape,
    frame=single
}

\renewcommand*{\footnoterule}{\rule{0 pt}{0 pt}}
\deffootnote[1.2 em]{1.2 em}{0 em}{\makebox[1.4 em][l]{\textbf{\thefootnotemark}}}

\newcommand{\assign}{\leftarrow}
